An Analysis of Deep Reinforcement Learning Agents for Text-based Games

Text-based games(TBG) are complex environments which allow users or computer agents to make textual interactions and achieve game goals.In TBG agent design and training process, balancing the efficiency and performance of the agent models is a major challenge. Finding TBG agent deep learning modules' performance in standardized environments, and testing their performance among different evaluation types is also important for TBG agent research. We constructed a standardized TBG agent with no hand-crafted rules, formally categorized TBG evaluation types, and analyzed selected methods in our environment.

==> methodology.tex <==

\section{Reinforcement Learning Methods}

As text-based game agent training requires interaction with the game environment, most related research works are built under the Reinforcement Learning(RL) framework. Various RL methods have been applied, including game states and action interpretation, RL algorithms and reward functions. In this section, we introduce basic concepts of major methodologies and classify related works in an ontology (Figure \ref{ontology}) for reader's reference.
% The joint task should also expect to inherit most of the issues of each sub-task, and we find this is true. The mass of research appears in the joint task, and as such newer methods have not been tried previously in the sub-tasks.



\subsection{State Representation}
Under the Reinforcement Learning framework, a text-based game environment can be modelled as POMDP, and the agents do not have direct access to the game states. One of the challenges for solving text-based games, even for a human, is interpreting visible game features and choosing the correct data formation to represent the game's state as accurately as possible.

\subsubsection{Embedding only}
Research works like \cite{narasimhan2015language,he2015deep} only use word embedding sequences generated from game state text description as game representations. Pre-trained, and non-pretrained methods are adopted, which is discussed in the word embedding section. Some researchers also concatenate features like game file names as game state representations.
\subsubsection{Graph aided}
Graph has been widely used as a feature to solve problems in many fields, such as bioinformatics and computer vision. For text-based games like Textworld games, the game states can be accurately represented by the graph. The accurate graph representation is usually not accessible to game players. Using pretrained neural networks or hand-crafted rules, some researchers try turning game state text description and agent experience into knowledge graphs. Neural network architectures like GCN can encode the generated knowledge graph.  

\subsection{Action Space}
Action space flexibility describes a text-based game agent's ability to adapt to complex action text and action sets. Some agents can only cope with a small fixed action set, and others can deal with action text with varying lengths, large vocabulary, and complex combinations.
\subsubsection{Non-flexible}
Text-based game agents' deep learning models could be designed with a fixed output fit a small action set. For example, \cite{yuan2018counting} fixed their network output shapes to 2 and 5, to deal with a fixed 2*5 (10 different action choices in total) game action set. This design has different sets of neural network layer weights for different action choices, which could be beneficial to predict value more accurately for each action. Yet due to the network output size only fits a fixed group of actions, this design is hard to generalize to games with longer action text sentences and varying action choices.
\subsubsection{Flexible}
To deal with action text sentences with arbitrary length and larger vocabulary, agent neural network models could be designed to have only one output node to predict state-action values. This kind of model is designed to predict values for all available actions and choose one to act based on the policy. These models have a stronger ability to generalize to different games. Yet, it doesn't have other groups of weight trained for each action, which makes the training process harder than non-flexible type models.
\subsubsection{Template-based}
Research works such as \cite{zahavy2018learn,jain2020algorithmic} have text action templates based on human gameplay experience. They only use the deep learning model to predict appropriate words to fill in the text action templates. This model type shares the same generalization problem with the non-flexible type, and the whole template needs to be redesigned to generalize to different games. Also, these models will need human gameplay experience to determine the most suitable text templates.


\subsection{Reinforcement Learning Algorithm}
Reinforcement Learning frameworks such as policy gradient, Q-learning and Actor-Critic are widely adopted in game solving and bioinformatics fields. \cite{narasimhan2015language} firstly adopted Deep Q-Learning to solve text-based games, and some following works adopted the same framework. Actor-critic is a widely used algorithm in recent years and has been successfully applied to complex problems like Go game.

\subsubsection{Deep Q-Learning}
Deep Q-learning(DQN) is a less complex yet powerful Reinforcement Learning algorithm. DQN is widely used in solving games like Atari. Q-learning uses the below function to update Q value and solve the game by approximating the Q value for each state.
\begin{equation}
Q_(s_{t},a_{t}) = \gamma\max_{a_{t+1}}Q(s_{t+1},a_{t+1})+r_{t}
\end{equation}

where $s_{t},a_{t},r_{t}$ demotes state,action and reward at time step $t$. 

For the text-based games field, \cite{narasimhan2015language} firstly adopted DQN to approximate the Q value for state-action and state-object pairs and select optimal pairs as the input for each text game state description. \cite{yuan2018counting} also used DQN, and their result showed that, with some additional reward design, DQN could support the text-based games to solve complicated games and generalize the performance on unseen games.


\subsubsection{Actor-Critic}
Actor-critic is considered a more advanced algorithm than DQN, and its capability has been proven to solve very complex games such as the GO game. Researchers have used Advantage Actor Critic(A2C) to train text-based game agents. A2C use below formula to calculate value \(v(s_{t})\) ,return \(R(s_{t},a_{t}) \) and advantage \(Adv(s_{t},a_{t}) \)for game states and actions. 
\begin{equation}
R(s_{t},a_{t}) = \gamma^{l}v(s_{t+l})+\sum_{k=1}^{l} \gamma^{k-1}r_{t+k}\
\end{equation}
\begin{equation}
Adv(s_{t},a_{t}) = R(s_{t},a_{t})-v(s_{t})
\end{equation}
 
 A2C is considered a reliable agent training method as it reduces variances using advantage. Yet most TBG research work doesn't compare performance between applying Q-learning and A2C, as it requires neural network architecture change.


\subsubsection{Reward Functions}

The goal of a Text-based game agent is to collect game scores from the environment as much as possible. A game score can be directly adapted as a reward to the agent. Researchers also designed reward functions to encourage certain agent behaviours, such as choosing actions likely to lead the agent to unexplored game states. For example, the exploratory reward function designed by \cite{yuan2018counting} encourages the agent to explore unseen states. 



%In this section we give an overview of papers which focused on the joint task itself, measuring their efficacy largely on performance against state-of-the-art. Generally they are using new technologies as they became available, or new architectures to make the learning more explicit. 





\section{Deep Learning Architectures and modules} \label{sec joint}

\subsection{Encoder Type}
As text-based game agents need to process text information given by game environment, the architecture of the text encoder type have a large influence on agent performance. The agent model also needs to be lite, as the agents are trained by sampling from game environments, and the text encoder needs to be efficient enough to support agent exploration.

\subsubsection{MLP}
Multilayer Perceptron(MLP) is a feed-forward neural network consisting of an input layer, one or more hidden layers and an output layer. MLP is a basic form of neural network and is widely used in domains like classification, regression and reinforcement learning. \cite{he2015deep} uses MLP to encode text inputs in TBGs. For each state/action text pair, DRRN\cite{he2015deep} feeds the state embedding vectors and action embedding vectors into two MLPs separately, then approximate the Q value based on the inner product of vectors from the last hidden layers of both MLPs.
\subsubsection{CNN}
Because of its outstanding performance in deep learning, Convolutional Neural Network(CNN) has become one of the most popular neural networks. Although CNN is more popular in computer vision, its performance in other domains like time series prediction and signal identification is also noticeable. The basic architecture of CNN includes an input layer, convolutional layers, pooling layers, fully-connected layers and an output layer. Various CNN models like VGGNet\cite{simonyan2015deep}, GoogLeNet\cite{szegedy2015going} and ResNet\cite{he2015deep} differ in the number of layers, number and size of kernels, etc.. For TBG tasks, \cite{zahavy2018learn,yin2019comprehensible,yin2020learning,yin2019learn} leverage CNN to encode game description text input. All the models are modified based on \cite{kim-2014-convolutional}. \cite{zahavy2018learn,yin2019comprehensible} use the similar CNN structure in \cite{kim-2014-convolutional}. \cite{yin2020learning,yin2019learn} only use a lite version of CNN, which consists of an input layer, Convolutional layer and max-pooling layer. The output of the max-pooling layer is the encoding of text input. Besides, \cite{yin2019comprehensible,yin2019learn,yin2020learning} add position embedding into CNN input to assist model learning.
\subsubsection{LSTM/GRU}
A recurrent Neural Network(RNN) is widely used in processing sequential data. It is commonly used in tasks, like machine translation, sentiment analysis, video analysis, speech recognition, etc. Long Short-Term Memory(LSTM) and Gated Recurrent Unit(GRU) are two typical forms of RNN. The input of both LSTM and GRU is word embedding, and each cell generates an output and a hidden state passed to the next cell. Research works such as\cite{narasimhan2015language,yuan2018counting} tokenize game state description text, map one-hot embeddings to higher dimensional word embedding sequences, and use LSTM to encode the embedding sequence as state encoding. Other works such as \cite{adolphs2020ledeepchef,hausknecht2020interactive} utilize GRU. Both output of LSTM/GRU and the hidden state of the last cell can be used as the game state encoding. 
\subsubsection{Transformer}
Since Transformer\cite{vaswani2017attention} was proposed, it has quickly become the hot field in research because of its great success. Although the original transformer is designed for NLP tasks, variants of transformers have entered other domains like computer vision and audio processing. The transformer in \cite{vaswani2017attention} has an encoder and a decoder. Both encoder and decoder take the word embedding sequence generated from game state text, and then add positional embedding onto the word embedding sequence. This sequence is used as the transformer encoder input. For TBG field, in\cite{adhikari2020learning}, \cite{yuan2019interactive} and \cite{yin2020learning} use transformer encoder to encode game state description text, and use the transformer encoder output as state or action encoding.
\subsubsection{BERT}
Bidirectional Encoder Representations from Transformers(BERT)\cite{kenton2019bert} is a pre-trained transformer-based model. It achieves many state-of-art performances in NLP tasks. In the TBG research field, research works like\cite{nahian2021training,yin2020learning} use BERT for state description text encoding. In these works, part of the weights of the encoder is frozen, and only a small part of the encoder layers will be fine-tuned during training, which makes the training more efficient. Compared to the Transformer encoder, the pre-trained BERT model normally uses it's own tokenizer and produces word segment embeddings. It has a much more number of parameters to capture information from a huge corpus. Among all the encoder types, BERT is the heaviest model.
\subsection{Word Embedding}


Word embeddings are used to represent tokens in given texts. Word embeddings can be pre-trained from the selected corpus and fixed for later use. Researchers sometimes unfreeze pretrained embedding weights to let downstream tasks update them. Most text-based game agents use embedding sequences to represent the game state or action text.

\subsubsection{Pretrained}
\cite{adhikari2020learning}, \cite{yuan2019interactive},\cite{nahian2021training} and \cite{yin2020learning} leverage pre-trained word embedding models and keep the embeddings fixed during training the agent. Among them, \cite{adhikari2020learning} and \cite{yuan2019interactive} use fastText\cite{mikolov2018advances}, \cite{yin2020learning} use Glove\cite{pennington2014glove} and BERT, \cite{nahian2021training} use BERT. \cite{jang2020monte} use spaCy\cite{Honnibal_spaCy_Industrial-strength_Natural_2020} which is a NLP library that provides static pre-trained word embeddings. In addition, \cite{he2015deep} uses bag-of-words(BOW), \cite{narasimhan2015language} compares BOW and bag-of-bigrams(BI) representation with trained LSTM embedding. \cite{yao2021reading} uses hash values as word embedding and shows the agent can achieve a high score even without language semantics.
\subsubsection{Non-pretrained}
Most of the agents discussed in this paper either fine-tune the pre-trained word embeddings or train the embeddings from scratch. Research works like \cite{narasimhan2015language}, \cite{yuan2018counting} initialize the word embeddings as either zeros or random vectors. Some research works like \cite{yao2021reading} and  \cite{murugesan2020enhancing} initialize the embedding using pre-trained Glove model, \cite{zahavy2018learn} uses word2vec\cite{mikolov2013efficient} model instead. Based on the experiment from \cite{yin2020learning}, although fully fine-tuning BERT outperforms freezing it during training, the former sacrifices the latter's advantage in training speed. \cite{yao2020keep} conducts similar experiments, and they compare fine-tuning pre-trained GPT-2\cite{radford2019language}---a model that only consists of decoder part of transformer---and learning a random initialized GPT-2, the result shows pre-trained GPT-2 has better performance.




\subsection{Pretrained Modules}
Pretrained modules are widely used in text-based game agent designs. With pretrained modules, text-based game agents are initialized with knowledge before exploring game environments. Using pretrained modules can improve agent performance, yet potentially could damage agent efficiency and generalization ability towards different games.
\subsubsection{Supervised}
\cite{ammanabrolu2019playing} trains a paired question encoder and answer encoder using DrQA\cite{chen2017reading} method. The data are generated from an agent that is accessible to the shortest solution of the game. The weights of the encoders and the embedding learned are used to initialize the agent. Ammanabrolu et al.\cite{ammanabrolu2019playing} only tested this method on TextWorld games with a 'home' theme in this paper. Later, they extended the question-answering pairs to a set of Jericho games and proposed Jericho-QA\cite{ammanabrolu2020avoid}. In 
this paper, Ammanabrolu et al.\cite{ammanabrolu2020avoid} pre-trained ALBERT\cite{lan2019albert} with Jericho-QA. The information extracted by ALBERT from text observation is used to update the knowledge graph during training. \cite{adolphs2020ledeepchef} pre-trained a task-specific module called Recipe Manager. It is used to predict what's left to complete the tasks. As mentioned, it can only be used in the cooking games generated by TextWorld. \cite{yao2020keep} pre-trains CALM with ClubFloyd\footnote{\url{http://www.allthingsjacq.com/interactive_fiction.html}---a dataset containing state-action pairs of TBGs--- to generate a relatively small size of possible actions at each turn of the game. 
\subsubsection{Unsupervised}
\cite{adhikari2020learning} proposed two methods to pre-train knowledge graph updater, which are Observation Generation (OG) and Contrastive Observation Classification (COC). OG trains the graph updater with a decoder to reconstruct text observation. COC instead trains the model to differentiate between true observation and a fake one.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{ontology2.png}
    \caption{ontology}
    \label{figure:ontology}
\end{figure}

% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=\linewidth]{ontology2.png}
%     \caption{Average scores for Transformer encoder with different embedding types}
%     \label{figure:ontology}
% \end{figure*}


% \begin{figure}
% \begin{tikzpicture}[grow'=right,level distance = 3.1in,sibling distance=.25in,scale=0.6]
% \tikzset{
%   treenode/.style = {shape=rectangle, rounded corners,
%                      draw, align=center,
%                      top color=white, bottom color=blue!20,level distance = 1in},
%   edge from parent/.style= 
%             {thick, draw, edge from parent fork right},
%   root/.style     = {treenode, font=\Large, bottom color=red!30,level distance = 1in},
%   l1/.style      = {treenode, font=\ttfamily\normalsize,level distance=1in, minimum width=1.1in,text width=0.9in, bottom color=orange!10,level distance = 1in},
%   l2/.style      = {treenode, font=\ttfamily\normalsize, minimum width=1.0in,text width=0.9in, bottom color=orange!20,level distance = 1in},
%   l3/.style      = {treenode, font=\ttfamily\normalsize, minimum width=3in,text width=3in, bottom color=orange!50}
%   %       every tree node/.style=             {draw,minimum width=1in,text width=1in,align=center}
%   }


\begin{figure}
\begin{tikzpicture}[grow'=right, level distance=3.3in, sibling distance=.25in,scale=0.4,
treenode/.style = {shape=rectangle, rounded corners,
                     draw, align=center,
                     top color=white, bottom color=blue!20,inner sep=10pt},
  edge from parent/.style= 
            {thick, draw, edge from parent fork right},
  root/.style     = {treenode, font=\Large, bottom color=red!30},
  l1/.style      = {treenode, font=\ttfamily\normalsize, minimum width=1.1in,text width=0.9in, bottom color=orange!10},
  l2/.style      = {treenode, font=\ttfamily\normalsize, minimum width=1.0in,text width=0.9in, bottom color=orange!20},
  l3/.style      = {treenode, font=\ttfamily\normalsize, minimum width=3.0in,text width=3.0in, bottom color=orange!50}
  %       every tree node/.style=             {draw,minimum width=1in,text width=1in,align=center}
  ]

  
  
\Tree 
    [. \node[root] {Model Features}; 
        [. \node [l1] {Encoder Type};
            [. \node[l2] {MLP};
              [. \node[l3] {\cite{he2015deep}};
              ]
            ]
            [. \node[l2] {CNN}; 
              [. \node[l3] {\cite{zahavy2018learn,yin2019comprehensible,yin2020learning,yin2019learn}};
              ]
            ]
            [. \node[l2] {LSTM/GRU}; 
              [. \node[l3] {\cite{narasimhan2015language,yuan2018counting,ammanabrolu2019playing,jain2020algorithmic,adolphs2020ledeepchef,hausknecht2020interactive,ammanabrolu2019graph,xu2020deep2,ammanabrolu2020avoid,murugesan2020enhancing,ammanabrolu2021learning,murugesan2021efficient,yao2020keep,yin2020learning,yin2019learn,jang2020monte,yao2021reading}};
              ]
            ]
            % [. \node[l2] {GRU}; 
            %   [. \node[l3] {\cite{adolphs2019ledeepchef,hausknecht2020interactive,ammanabrolu2020graph,ammanabrolu2020avoid,murugesan2020enhancing,ammanabrolu2021learning,murugesan2021efficient,yao2020keep}};
            %   ]
            % ]
            [. \node[l2] {Transformer}; 
              [. \node[l3] {\cite{adhikari2020learning,yuan2019interactive,nahian2021training,yin2020learning}};
              ]
            ]
        ]
        [. \node [l1] {Word Embedding};
            [. \node[l2] {Pretrained};  
              [. \node[l3] {\cite{narasimhan2015language,he2015deep,adhikari2020learning,yuan2019interactive,nahian2021training,yin2020learning,jang2020monte,yao2021reading,ammanabrolu2021learning}};
              ]
            ]
            [. \node[l2] {Non-pretrained}; 
              [. \node[l3] {\cite{narasimhan2015language,zahavy2018learn,yuan2018counting,ammanabrolu2019playing,jain2020algorithmic,adolphs2020ledeepchef,hausknecht2020interactive,ammanabrolu2019graph,xu2020deep2,ammanabrolu2020avoid,murugesan2020enhancing,yin2019comprehensible,yao2020keep,yin2020learning,yin2019learn,jang2020monte,yao2021reading}};
              ]
            ]
        ]
        [. \node [l1] {RL Frame Work};
            [. \node[l2] {DQN}; 
              [. \node[l3] {\cite{narasimhan2015language,he2015deep,zahavy2018learn,yuan2018counting,ammanabrolu2019playing,jain2020algorithmic,hausknecht2020interactive,adhikari2020learning,yin2019comprehensible,yuan2019interactive,yao2020keep,yin2020learning,yin2019learn,jang2020monte,yao2021reading}};
              ]
            ]
            [. \node[l2] {Actor-Critic}; 
              [. \node[l3] {\cite{adolphs2020ledeepchef,ammanabrolu2019graph,xu2020deep2,ammanabrolu2020avoid,murugesan2020enhancing,ammanabrolu2021learning,murugesan2021efficient,nahian2021training}};
              ]
            ]
        ]
        [. \node [l1] {Action Space Flexibility};
            [. \node[l2] {Non-flexible}; 
              [. \node[l3] {\cite{narasimhan2015language,zahavy2018learn,yuan2018counting,yuan2019interactive}};
              ]
            ]
            [. \node[l2] {Flexible}; 
              [. \node[l3] {\cite{he2015deep,ammanabrolu2019playing,jain2020algorithmic,adolphs2020ledeepchef,adhikari2020learning,ammanabrolu2021learning,yin2019comprehensible,murugesan2021efficient,yao2020keep,nahian2021training,yin2020learning,yin2019learn,jang2020monte,yao2021reading}};
              ]
            ]
            [. \node[l2] {Template based}; 
              [. \node[l3] {\cite{adolphs2020ledeepchef,hausknecht2020interactive,ammanabrolu2019graph,ammanabrolu2020avoid,murugesan2020enhancing}};
              ]
            ]
        ]
        [. \node [l1] {State Representation};
            [. \node[l2] {Graph-aided}; 
              [. \node[l3] {\cite{ammanabrolu2019playing,ammanabrolu2019graph,adhikari2020learning,ammanabrolu2020avoid,murugesan2020enhancing,ammanabrolu2021learning,murugesan2021efficient}};
              ]
            ]
            [. \node[l2] {embedding only}; 
              [. \node[l3] {\cite{narasimhan2015language,he2015deep,zahavy2018learn,yuan2018counting,jain2020algorithmic,adolphs2020ledeepchef,hausknecht2020interactive,yin2019comprehensible,yuan2019interactive,yao2020keep,nahian2021training,yin2020learning,yin2019learn,jang2020monte,yao2021reading}};
              ]
            ]
        ]
        [. \node [l1] {Pretrained Module};
            [. \node[l2] {Supervised};
              [. \node[l3] {\cite{ammanabrolu2019playing,adolphs2020ledeepchef,ammanabrolu2020avoid,yao2020keep}};
              ]
            ]
            [. \node[l2] {Unsupervised}; 
              [. \node[l3] {{\cite{adhikari2020learning,ammanabrolu2021learning}}};
              ]
            ]
        ]
    ]
\end{tikzpicture}
\caption{Ontology for TBG agent methods}
\label{ontology}

\end{figure}




